Before Reasoning Can Fail: Pre-Evidence Procedural Failures in Agentic RAG

Agentic retrieval-augmented generation (RAG) systems can fail before evidence-conditioned reasoning is tested: an agent may retrieve candidate snippets but finalize without inspecting them. We study this failure mode as a procedural property of the agent trajectory, decomposing wrong answers into pre-evidence discipline failures and post-gold-read failures using saved tool-call traces, retrieved evidence, read passages, and final answers. Across 12,000 paired trajectories on HotpotQA, 2WikiMultiHopQA, and MuSiQue, the two failure types are largely non-redundant: the both-trigger rate is in [11.2%, 13.1%] across regex and spaCy entity extractors. We then evaluate Read-Gate, a minimal runtime invariant requiring an agent to read after search and before finalization. Forced reading improves LLM-Acc by 14.9-19.9 points on trajectories that would otherwise skip reading and by 3.2-9.4 points on full minimal-reasoning cells. Additional diagnostics show that larger hidden thinking budgets do not necessarily increase evidence inspection. Together, these results indicate that evidence-gathering should be evaluated as a trajectory-level control problem, separately from answer-side reasoning.

==> sections/06_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

The experiments suggest that procedural discipline is a separate engineering lever from reasoning effort. Scaling the reasoner can improve answer synthesis after evidence has been read, but it does not guarantee that the agent executes the external evidence-gathering procedure. \rg should therefore be interpreted as a diagnostic intervention rather than a universally optimal control policy: it helps when residual discipline error is high, but has little headroom when the agent already reads reliably. More broadly, final-answer accuracy alone merges distinct failure regimes. A wrong answer after reading evidence and a wrong answer produced before evidence inspection may receive the same correctness label, but they require different interventions. This is the central role of trajectory-level evaluation: it makes evidence inspection measurable rather than implicit.

We observe non-monotone discipline behavior across model and effort regimes (gpt-4o-mini $7.6\%$, gpt-5-mini minimal $13.3\%$, gpt-5-mini medium $4.5\%$ on HotpotQA), suggesting that stronger parametric capacity does not monotonically improve procedural compliance. We leave the mechanism to future work.

\paragraph{Tool-channel framing.}
The mechanism ablation (\S\ref{sec:exp-mechanism}) suggests that the channel through which evidence is delivered can affect whether the agent uses it for grounding. In our HotpotQA ablation, delivering the same chunk text as a \texttt{user}-role observation recovers only a minority of \rg's gain, and qualitative disagreement cases include responses in which the agent treats the injected text as conversational side information (\emph{``Thanks --- do you want me to re-evaluate?''}) rather than as evidence to commit to. We interpret this as suggesting that tool-mediated inspection contributes to grounding beyond token-level access alone; the mechanism scope here is HotpotQA / gpt-5-mini-minimal, and broader tool-channel effects across tasks and backbones remain open.
